Detecting DBMS Bugs with Context-Sensitive Instantiation and Multi-Plan Execution

DBMS bugs can cause serious consequences, posing severe security and privacy concerns. This paper works towards the detection of memory bugs and logic bugs in DBMSs, and aims to solve the two innate challenges, including how to generate semantically correct SQL queries in a test case, and how to propose effective oracles to capture logic bugs. To this end, our system proposes two key techniques. The first key technique is called context-sensitive instantiation, which considers all static semantic requirements (including but not limited to the identifier type used by existing systems) to generate semantically valid SQL queries. The second key technique is called multi-plan execution, which can effectively capture logic bugs. Given a test case, multi-plan execution makes the DBMS execute all query plans instead of the default optimal one, and compares the results. A logic bug is detected if a difference is found among the execution results of the executed query plans. We have implemented a prototype system called Kangaroo and applied it to three widely used and well-tested DBMSs, including SQLite, PostgreSQL, and MySQL. Our system successfully detected 50 new bugs. The comparison between our system with the state-of-the-art systems shows that our system outperforms them in terms of the number of generated semantically valid SQL queries, the explored code paths during testing, and the detected bugs.

==> 11-backup.tex <==
\subsection{Parser Generation}
To help understand our parser generation, we introduce the syntactic rules of the parser first.
The parser's process contains lexical analysis and syntax analysis.
The lexical analysis scans the input and returns a stream of tokens handled by Bison~\cite{Bison}. 
% Each token contains two parts, the token and its value.
The syntax analysis typically turns a sequence of tokens into a parse tree to figure out the relationship among the input tokens.
The syntactic rules define how to create a branch in the parser tree. 
In other words, each matched syntactic rule usually maps to a parse tree node.

The Bison syntactic rules have the general form: \code{target\_symbol : components…;}.
The \code{target symbol} describes the target of this rule, and \code{components} are the detailed rules.
Multiple rules for the same target symbol can be joined with the character \code{|}.
For example, \code{expr: expr ADD expr | CONST } claims two syntactic rules.
The first one defines that two \code{expr} can be
combined together with a \code{ADD} to generate a new symbol \code{expr}.
The second one implies a \code{CONST} token is also a symbol \code{expr}.
Each syntactic rule can accompany an \code{action} that contains C language source code surrounded by braces, 
which will be executed when the rule is matched.
The C action code goes in braces at the end of each rule. Each symbol and token in a bison rule has a value. 
The value of the target symbol (the one to the left of the colon) is called "\$\$" in the action code, and the values on the right are numbered "\$1", "\$2", and so forth, up to the number of symbols in the rule.

Figure \ref{fig:parser_generator} shows an example of how to automatically generate the parser from the grammar rule files.
To generate an accurate parser, we first collect the token list and syntax structure which are well structured in DBMS Bison files.
Then, we fill in all the action codes.
In our fuzzer mutator, the parse tree serves as a data structure for later use, such as translating the tree back to SQL string or doing some mutation on the tree nodes.
In order to achieve these goals, the action code should record the sequence of operations the parser does and the token values.
The generated AST node file defines all possible node types which are used to record the specific branch information and token values.



Most open-source relational DBMSs utilize Bison~\cite{Bison} to build their parsers, such as MySQL, PostgreSQL, MariaDB, and TiDB.
Though our prototype is Bison-specific, this approach can also be easily adapted to other parser generator tools if they also follow BNF.


\begin{figure}[t]
\centerline{\includegraphics[width=0.49\textwidth]{Fig/generator.png}}
\caption{An example to show the process of AST-based mutator generation.}
\label{fig:parser_generator}
\end{figure}

The flex is responsible for lexical analysis, which scans the input and returns a stream of tokens handled by Bison. Each token contains two parts, the token and the token's value.
The flex rule file of \ref{fig2} contains two regular expression patterns, and each pattern is followed by the C code(in braces \code{\{\}}) to execute when the pattern matches.
The first one matches an operator \code{"+"} and returns a token \code{ADD}.
The second one,\code{"[A-Za-z0-9]+"} is a regular expression used to match an identifier. In flex action code, the variables\code{yytext}is set to point the input text that the pattern just match, and the variables\code{yyval} stores the token values.
Specifically, it saves the string into the token values and return a token\code{IDENT}. 
We call a token with a fixed value a fixed token (.e.g\code{ADD}), otherwise, we call it a variable token (.e.g\code{IDENT}).

The bison use BNF to describe the rules that turn a series of tokens into a parse tree to figure out the relationship among the input tokens. 
It mainly contains three parts: a token list, a set of rules that define how to create a branch of the parse tree, and the action codes when a rule is matched.
% In some applications, it creates the tree as a data structure in memory for later use. In others, the tree is just implicit in the sequence of operations the parser does. 
In the example, the first two lines of the bison rule file declare the tokens get from flex. Following that are four BNF rules.
The name on the left side of \code{":"} (\code{expr} and \code{column\_ref}) is a symbol called target symbol and the right of \code{"|"} indicates a way to create a branch of this symbol.
For example, the first rule, which define the symbol \code{expr}, means that an \code{expr} is a \code{column\_ref}. The second rule \code{expr ADD expr} means that an \code{expr} might be an addition expression where its left and right operands are both an \code{expr}.
% With rules that refer to themselves directly or indirectly, these simple rules can match an arbitrarily complex sequence of additions.
Again, like flex, the C action code goes in braces at the end of each rule. Each symbol and token in a bison rule has a value. 
The value of the target symbol (the one to the left of the colon) is called "\$\$" in the action code, and the values on the right are numbered "\$1", "\$2", and so forth, up to the number of symbols in the rule.
% The values of the tokens are stored in \code{yyval} when flex returned the token.  
In the following, we refer to these BNF rules as syntax structures.

To generate an accurate parser, we first collect the token list and syntax structure which are well structured in DBMS flex/bison files.


Then, we fill the action code for all rules in the bison file.
In our fuzzer mutator, the parse tree serves as a data structure for later use, such as translating the tree back to SQL string or doing some mutation on the tree nodes.
In order to achieve these goals, the action code should record the sequence of operations the parser does and the token values.
The generated AST node file defines all possible node types which are used to record the specific branch information and token values.
% The AST node file is written in C++ and each class defines an AST node type for the target symbol. 
% We generate an AST node file that defines all possible AST nodes to record the branch information and token values.
% We generate an AST node file that defines all possible AST node class to record the branch information and token values.
Specifically, for each action code of the rule, we first create an AST node of the corresponding type for the target symbol.
Then store the values of the token and the nodes of symbols on the right inside this AST node. 
% Specifically, we assigned each target symbol with a specific value type which serves as an AST node type. 
In addition, we use an \code{id\_} to identify which rule is used to create this target symbol. Note that only the values of symbols and variable tokens will be stored in the AST node, because the fixed token and their values can be inferred from \code{id\_}.
% For instance, target symbol \code{expr} has a node \code{class Expr} which has three branch \code{column\_ref\_}, \code{expr\_1\_}, and \code{expr\_2\_}.



% \subsection{Case Studies on Detected Bugs}
% We provide several cases studies to show the security impact of logic bugs and MPE's contribution to detecting memory bugs.

% \begin{lstlisting}[language=sql,float=t,
% label={list:dynamic_constraints},
% numbers=left,
% numbersep=2pt,
% xleftmargin=1em, 
% commentstyle=\color{codegreen},
% backgroundcolor=\color{mygray},
% basicstyle=\footnotesize\ttfamily,
% keywordstyle=\color{purple},
% % keywordstyle=\bfseries,
% breaklines=true,
% numberstyle=\ttfamily,
% caption={An example shows the dynamic semantic constraints in SQL. DBMS will check the values of column \code{b} in table \code{t2} to satisfy the condition \code{b>1} during the execution.} ]
% CREATE TABLE t1(a INT CHECK(a>1));
% INSERT INTO t1 SELECT b FROM t2;
% \end{lstlisting}

% \begin{table}[t]
% \scriptsize
% \caption{The types of semantic constraints.} % title of Table
% \centering % used for centering table
% \setlength{\tabcolsep}{0.48mm}{
% \begin{tabular}{l c} % centered columns (4 columns)
% \toprule %inserts double horizontal lines
% Constraint Type & Example  \\  % inserts 
% \hline % inserts single horizontal line
% Variable type & ${\scriptstyle Type(a)=TableRef; Type(b)=ColumnId}$  \\
% Data type & ${\scriptstyle DataType(a)=STRING; DataType(a)!=DataType(b)}$ \\
% Name & ${\scriptstyle Name(a)!=Name(b); UniqueName(a\in A)}$ \\
% % Name & ${\scriptstyle Name(a)!=Name(b); UniqueName(a\in A) \;is \; unique\; in\; the\; set\; A}$ \\
% Attribute & ${\scriptstyle Attr(b)!=(GENERATED); AttrX(a)=AttrX(b)}$ \\
% Value & ${\scriptstyle a\in\{1, 2, 3...\}; b\in[x, y]}$  \\
% Dependency & ${\scriptstyle a\in\{v1, v2...\}; a\in T | T\in\{t1, t2...\} }$  \\
% Distinct & ${\scriptstyle DISTINCT[a, b, c, d] }$ \\
% Composite & ${\scriptstyle (DataType(a), DataType(b))\in\{(bool, numeric),...\} }$ \\
% %heading11
% \bottomrule
% \end{tabular}}
% \label{smenaitc-constraint-type} % is used to refer this table in the text
% \end{table}


% This table shows the semantic type, an example statement constains that type of semantic constraint, and the function of that semantic constraint.
% \subsection{Semantic constraints examples}



% \begin{table*}[th]
% \scriptsize
% \caption{Semantic constraints example. This table shows the semantic type, as well as an example statement, that contains such type of constraint.} % title of Table
% \centering % used for centering table
% \setlength{\tabcolsep}{0.48mm}{
% \begin{tabular}{l|l|l|l} % centered columns (4 columns)
% \toprule %inserts double horizontal lines
% Constraint Type & Example SQL & Example Constraint & Explain \\ 
% \hline
% Variables type & SELECT * FROM x1 ORDER BY i1; & ${\scriptstyle Type(i1)=ColumnId}$ & i1 is a constant with type ColumnId \\
% Data type & SELECT x1+1 FROM x2; & ${\scriptstyle DataType(x1)=numeric}$ & The data type of column x1 should be numeric \\
% Name & SELECT x1 FROM x2; &  ${\scriptstyle UniqueName(x1\in x2)}$ & x1 is a column with unique name in table x2 \\
% Attribute & INSERT INTO x1(x2) VALUES (i1); & ${\scriptstyle Attr(x2)!=GENERATED}$ & x2 should not be a generated column \\
% Value & SELECT * FROM x1 ORDER BY i1; & ${\scriptstyle i1\in\{1, 2, ..., Size(x1)\}}$ & i1 is an integer up to the number of columns of table x1 \\
% Dependency & SELECT x1 FROM (SELECT x2, x3 FROM x4) AS x5; & ${\scriptstyle x1 \in \{x2, x3\}}$ & x1 could be column x2 or x3 \\
% Distinct & INSERT INTO x1(x2, x3) ...; & ${\scriptstyle DISTINCT[x2, x3]}$ &  x2 and x3 should be two different column \\
% Composite & SELECT (x1, x2) IN (TABLE x3) FROM x4; & ${\scriptstyle (DataType(x1), DataType(x2))) \in}$   & The data type of x2 and x3 should be \\
% & & ${\scriptstyle \{DataType(x3,1), DataType(x3,2)\}}$ & the same as the first two columns in table x3. \\
% %heading11
% \bottomrule
% \end{tabular}}
% \label{tab:constraint_example}
% \end{table*}
